VL-CheckList: Evaluating Pre-trained Vision-Language Models with Objects, Attributes and Relations

Vision-Language Pretraining (VLP) models have recently successfully facilitated many cross-modal downstream tasks. Most existing works evaluated their systems by comparing the fine-tuned downstream task performance. However, only average downstream task accuracy provides little information about the pros and cons of each VLP method, let alone provides insights on how the community can improve the systems in the future. Inspired by the CheckList for testing natural language processing, we exploit VL-CheckList, a novel framework to understand the capabilities of VLP models. The proposed method divides the image-texting ability of a VLP model into three categories: objects, attributes, and relations, and uses a novel taxonomy to further break down these three aspects. We conduct comprehensive studies to analyze seven recently popular VLP models via the proposed framework. Results confirm the effectiveness of the proposed method by revealing fine-grained differences among the compared models that were not visible from downstream task-only evaluation. Further results show promising research direction in building better VLP models. Our data and code are available at: https://github.com/om-ai-lab/VL-CheckList.

==> analysis.tex <==
First, we show that how easy negative sample achieve high performance across all models on in-domain datasets such as COCO, GCC, SBU, and VG. However, when we apply easy negative samples from out-of-domain corpus. The performance drops significantly 





==> bak-intro.tex <==

We found the following issues when evaluating VLP models as well:.
\begin{itemize}
\item Benchmark images and pre-training images are overlapped
\item Most benchmark evaluation is on downstream tasks. We evaluated the pretraining model itself using ITM and ITC heads and downstream tasks and comparing correlation.
\item it is expensive to train all downstream tasks for evaluating VLP models. 
\item it is ambiguous to tell the performance is because of the pre-trained model or 
downstream objectives. 
\end{itemize}

To improve the robustness of a VLP model, we can apply the generalization technique on both vision and text modalities. In the vision, image augmentation is the most well-known method to improve the generalization ability. Most work excludes color inversion because texts often contain color information, cutout, some important small objects could be cut out. In the text side, a various negative sampling strategy has been conducted to distinguish confusing examples. However, most studies applied simple random negative sampling without considering various linguistic variations. For example, a model predicts "car" in the picture. However, it often fails to predict a specific color "a red car" or a number "three cars" or a position "in front of the car". 

In this paper, we propose VL-CheckList, which easily evaluates various aspects of VLP models with linguistic capabilities. 
VL-CheckList guides users in what to test, by providing a list of linguistic capabilities, which are applicable to most tasks. VL-CheckList helps users to understand the model capability and robustness.



Probing Image-Language Transformers for verb understanding
Testing the quality of the pretrained representations - in particular, if these models can distinguish different types of verbs or if they rely soly on nouns in a given sentences. Their goal is to investigate if the good performance of these models is due to leaned representations that successfully relate different aspects of language to images. They found that the models fail more in situations that require verb understanding compared to other parts of speech.  

An Empirical Study of Training End-to-End Vision-and-Language Transformers
They investigate how to design and pre-train a fully transformer-based VL model in an end-to-end manner. Specifically, they dissect the model designs along multiple dimensions: vision encoders (e.g., CLIPViT, Swin transformer), text encoders (e.g., RoBERTa, DeBERTa), multimodal fusion module (e.g., merged attention vs. co-attention), architectural design (e.g., encoder-only vs. encoder-decoder), and pre-training objectives (e.g., masked image modeling). 

Decoupling the role of data, attention, and losses in multimodal transformers
They investigated the tree important factors which can impact the quality of learned representatiosn: pretraining data, the attention mechanism, and loss function


Propose a model-agnostic and task-agnostic testing methodology that 
tests individual capabilities of the model . They revealed critical bugs in commercial developed by large software companies, making it easy to incorporate in current benchmarks or evaluation pipelines. only in natural language processing model, not in multimodal setting. 


==> baselines.tex <==

In this session, we describe the existing VLP models that we included in our model analysis. We have listed them below in chronological order of publications.  

\noindent\textbf{LXMERT: } %pub 2019 Aug @ 朱明炜
LXMERT is a model based on transformer architecture and consists of three encoders (based on transformer), an object relationship encoder, a language encoder, and a cross-modality encoder. The input of LXMERT is an image and sentence of description. Faster R-CNN is used to detect the target of the image, and the input sentence is divided into tokens by wordpiece tokenizer. The local features (ROI feature of 2048-dim) and the location information (bounding box) extracted from the image will be fused through the LN layer. The value of layer norm is used as input of the object relationship encoder.The value of word embedding (WordEmbed) and token index (IdxEmbed) are added through LN layer. Finally, the values of image and text encoder are used as the input of cross modality encoder to complete the interaction of cross modality information.The model outputs three results: including visual and text output and cross modality output. LXMERT did five different pre-training tasks. The image data in the pre-training stage is aggregated of different datasets. During the experiment, it is found that the experimental performance without data augment is better when pre-training or fine-tuning. Lxmert achieved SOTA on two image QA datasets (i.e., VQA and GQA). 

\noindent\textbf{UNITER: } %pub 2019 Sep @ 朱明炜
UNITER consists of an Image Embedder, a Text Embedder and a multi-layer Tran sformer, learned through four pre-training tasks: Masked Language Mo deling conditioned on image regions (MLM), Masked Region Modeling conditioned on input text (MRM), Image-Text Matching (ITM), and Word-Region Alignment (WAR). UNITER uses conditional masking operation on image and text respectively. On the premise of ensuring the integrity of one modal, mask information of another modal. In this way, we can better understand which modal has an impact on the performance of model itself. During the pretraining stage, Faster R-CNN is used to extract the image region features for coding processing, while retaining the position information of the local feature map, and both are encoded into the same embedding space together. On the other hand, the model uses tokenizer of the original BERT to segment sentences into tokens, also retaining the location information, and synthesize embedding with Text Embedder. The embedding of image and text is processed by LN layer respectively, and then the image and text features are joined as the input of transformer. Finally, a Transformer module is applied to learn contextualized embeddings for each region and each word. Each pair of negative samples in the model is randomly replaced by other data in the dataset (image or text). UNITER$_{base}$ and UNITER$_{large}$ models trained by in-domain and out-of-domain data. Through ablation experiments, the best combination of pre-training tasks are found to meet more downstream task scenarios.

\noindent\textbf{OSCAR: } %pub 2020 April @ 沈昊展
Oscar has no separate text encoder and image encoder. For image features, OSCAR introduces object tags detected from an image as anchor point to ease the learning of image-text alignment.On the one hand, Faster R-CNN is used to extract the visual semantics of given regions from an image, which includes both information of region feature and region position, then these two part will be concatenated to a position-sensitive region feature vector and be further transformed into final region vectors using a linear projection. On the other hand, the same Faster R-CNN is used to detect a set of high precision object tags.Then a triple (\textbf{\textit{w}}, \textbf{\textit{q}}, \textbf{\textit{v}}), where \textbf{\textit{w}} is the word embedding of the text, \textbf{\textit{q}} is the word embedding of the object tags, and \textbf{\textit{v}} is the set of region vectors of the image, is represented as the input of OSCAR. OSCAR is pre-trained with two objectives: optimizing \textit{Masked Token Loss} and \textit{Contrastive Loss} . OSCAR teams found that the \textbf{\textit{q}} and \textbf{\textit{w}} share the same linguistic semantic space, while \textbf{\textit{v}} lies in the visual semantic space, so they apply the Masked Token Loss(MTL) for pre-training: each token in [\textbf{\textit{w}}, \textbf{\textit{q}}] is randomly masked with probability 15\% and replaced with special token [MASK], the goal of training is to predict these masked tokens based on their surrounding tokens and all image features, which is similar to masked language model used by BERT.From another perspective, [\textbf{\textit{q}}, \textbf{\textit{v}}] can be considered as the image modality and \textbf{\textit{w}} as the language modality. As the result of it, authors sample a set of “polluted” image representations by replacing \textbf{\textit{q}} with probability 50\% with a different tag sequence randomly sampled from the same dataset, then the model is asked to predict whether the input is original representation or polluted one, which is the process of optimizing Contrastive Loss. OSCAR creates SoTA on six vision-language tasks, which shows that the learning of cross-model representation can be significantly improved by utilizing object tags detected from images.

\noindent\textbf{ViLT: } %pub 2021 Feb @ 沈昊展
Before being inputted into transformer block, the input text of ViLT is embedded to word embedding through a word embedding matrix and further summed with a position embedding matrix.Being different from the majority of common methods of vision encoding (e.g. region feature,grid feature), patch projection, the crucial element to make ViLT faster than other VLP models is used to generate visual embedding: the input image is sliced into patches, then embedded into visual embedding with a linear projection and position embedding.The text and image embeddings are summed with their corresponding modal-type embedding vectors, then are concatenated into a combine sequence, which is the 
final input for transformer module. There are two pre-training objectives in ViLT: image text matching (ITM) and masked language modeling (MLM). For ITM, authors randomly replace the aligned image with a different image with the probability of 0.5 and ViLT is asked to judge whether the image-text pair is matching. What's more, authors design word patch alignment(WPA) that computes the alignment scores between textual subsets and visual subsets. The objective of MLM is to predict the ground truth labels of masked text tokens from its contextualized information, which is similar to BERT. For the first time,ViLT achieves competent performance on vision-and-language tasks without using region futures or deep convolutional visual embedders in general, and it commissions the transformer module to extract and process visual features in place of a separate deep visual embedder, which leads to significant runtime and parameter efficiency. 


\noindent\textbf{CLIP: } %pub 2021 Feb @ 朱明炜
CLIP is trained on a dataset of 400 million (image, text) pairs collected from the internet, and implements efficient scalable classification model.Unlike the traditional end to end or region base model in the multimodal field, CLIP uses the strategy of metric learning.It contains two subjects: text and image encoder. Text encoder is used to extract text features. Text transformer model commonly used in NLP can be used. Image encoder is used to extract image features, and common CNN model or vision transformer can be used.In the pre-training stage, natural language is regarded as the inference supervision signal of visual information, and then the cosine similarity is calculated according to the image-text features.In the downstream test stage, the input is an image corresponding to N texts, and output is the predicted classification probability of N description texts. Furthermore, the model commonly used in CV is usually pre-trained and then fine-tuned.On the contrary,CLIP can directly achieve zero-shot image classification, that is, it does not require any training data to achieve classification on a specific downstream task.The experimental results of zero-shot CLIP on 16 datasets rival those of  ResNet-50.



\noindent\textbf{ALBEF: } %pub 2021 Jul @ 张天祺
ALBEF consists of a text encoder, an image encoder, and a multimodal encoder. The text encoder and multimodal encoder are both initialized with BERT$_{base}$ model. The former uses the first six layers of the BERT$_{base}$, while the latter uses the last six layers. The image encoder is a 12-layer visual transformer ViT-B/16, which is initialized with weights pre-trained on ImageNet-1k. ALBEF is pre-trained with three objectives: image-text contrastive learning (ITC) on the unimodal encoders, masked language modeling (MLM) and image-text matching (ITM) on the multimodal encoder. To sample hard negatives for the ITM task, the authors use the contrastive similarity to find in-batch hard negatives, which share similar semantics but have distinctions in fine-grained details. In addition, to learn better representations from noisy image-text pairs, the authors propose to learn from pseudo-targets produced by the momentum model. The highlight of ALBEF is the image-text contrastive learning (ITC) pre-training objective, which exerts great effects on the performance of model. ITC loss aims to align the unimodal representations of an image-text pair before fusing them through cross-modal attention, helping the model learn better unimodal representations before fusion.
%[1]:Devlin, J., M. Chang, K. Lee, et al. BERT: pre-training of deep bidirectional transformers for language understanding. In J. Burstein, C. Doran, T. Solorio, eds., NAACL, pages 4171–4186.2019.
%[2]:Dosovitskiy, A., L. Beyer, A. Kolesnikov, et al. An image is worth 16x16 words: Transformers for image recognition at scale. In ICLR. 2021.

\noindent\textbf{TCL: } %pub 2022 Feb @ 张天祺
TCL is improved on the basis of ALBEF, so the model architecture is basically consistent with ALBEF. Besides ITM and MLM tasks, TCL introduces three contrastive modules: cross-modal alignment (CMA), intra-modal contrastive (IMC), and local MI maximization (LMI), which respectively aims to maximize the mutual information between the matching image and text, maximizes the global mutual information between differently augmented views and maximizes mutual information between the global representation and local region. Rather than only perform cross-modal alignment, TCL fully utilize both cross-modal and intra-modal self-supervision. Additionally, compared with simply considering the influence of global information for multi-modal contrastive learning, TCL maximizes the mutual information between local regions and global representations to make use of localized and structural information from image and text input. For ITM task, authors generate negative examples through batch-sampling, which is same as ALBEF. It is worth emphasizing that TCL is the first work to consider local structure information for multi-modality representation learning.






==> discussion.tex <==
\subsection{Analysis on CLIP model}
In this section, we discuss the fastest degradation of CLIP performance in (Large to Small) and (Center to Margin), as well as the reasons for the poor results of Attribute:

\textbf{Center vs. Margin}:
From Table \ref{obj}, it can be seen that the gap score between Center and Margin of CLIP model is 11.87\%, which is one of the largest average contrast fluctuation among all models. Appendix Table \ref{clip_good} shows that the results of CLIP on SWiG and HAKE are good, but the results in VG dataset are poor. We guess that the CLIP model itself has limited ability to understand the semantic information of complex scenes. In the pre-trainning stage, it calculates the feature similarity according to a piece of text and an image, but region base model uses the external convolution architecture to extract region targets from images, and end-to-end model makes better use of attention mechanism to learn the similar fraction of image-text in the feature fusion stage. The above method, which is different from CLIP, may be better than calculating the similarity using the feature matrix alone. By contrast, in the aspects of cross modal feature fusion, attention mechanism can better insight into objects with smaller area. In order to test this hypothesis, we did an extension experiment of CLIP on the location-related datasets. Each data item of VG provides \textbf{'region-info'} label, including the bounding box of the image regions of \textit{subj} and \textit{obj}. Therefore, we integrate two bounding boxes into a matrix box, extract the image regions, and keep the description text in the sample unchanged to form a new image-text pair \textbf{(Image$_{local}$,text)}, and constructed variant datasets for VG: Local$_{subj}$, Local$_{obj}$. The results of the supplementary experiment are shown in Table \ref{clip_local} . We see that by removing as much of the edge information that is independent of the single-segment text description as possible from the image, the results of CLIP for local image on Local$_{subj}$ and Local$_{obj}$ are outperformed the original CLIP (no image region is extracted), 3.9\% and 5.7\% higher respectively. The results were even better than the region base multimodal models. The table \ref{obj} shows that multimodal models generally pay more attention to the central semantic information of images, which is similar to the perspective of human observation. Focusing on the image region will improve the ability of CLIP model to obtain more fine-grained visual signals. We believe that the sensitivity of CLIP to scene location information is a work worthy of further study.


\textbf{Large vs. Small}:
 We further measure how the pixel size of the region in the image will affect the model. The variance value of CLIP from the small and large region images is the largest, which is 13.13\% degradation. The region base and end to end models are more stable, even if the other six models are used for single comparison, the conclusion is still the same. This is not only due to the absence of attention mechanism in feature similarity computing. CLIP was trained to match an image as a whole to a text description, without capturing the fine-grained alignment between image regions and text spans, so the understanding of local information is not very good ~\cite{zhong2022regionclip}.
 
 \textbf{Poor Attribute}:
 Table \ref{attr} shows that the ability of CLIP to understand attribute related visual commonsense was poor, which is more prominent than other models. Whether it is the influence of neural network structure difference or the training data is also a work worth discussing in the future.
 
 
 
\begin{table}[ht]\centering    
    \begin{tabular}{c|c|c|c|c}
    \hline
    Model\ \textbf{\textbackslash{}}\ VG$_{data\_type}$ &Subj &Obj &Local$_{subj}$ &Local$_{obj}$\\
    \hline
    ViLT & \textbf{89.3}	&\textbf{95.1}	&-	&- \\
    ALBEF & 87.8	&93	&-	&- \\
    OSCAR & 83.9	&84.7	&-	&- \\
    UNITER & 84.8	&86.4	&-	&- \\
    LXMERT & 84.3	&86.8	&-	&- \\
    TCL & 85	&91.1	&-	&- \\
    CLIP & 80.7	&86	&-	&- \\
    CLIP\_Local & -	&-	&\textbf{84.6}	&\textbf{91.7} \\
    \hline
    \end{tabular}
    \caption{Subj and Obj are two attribute subsets extracted from VG dataset. Using the bounding box tag of VG to merge and extract the region image pointed by \textit{subj} and \textit{obj} fields, a new dataset is constructed. The text remains the same as previous content \textbf{(Image$_{local}$,text)}. It only does the expansion experiment for CLIP.}
    \label{clip_local}
\end{table}



==> exp-backup.tex <==

\noindent\textbf{VG: }
Visual Genome (VG) is aimed to help models develop a
broader understanding of our visual world and capacities to detect objects with abilities
to describe objects in a image and explain their interactions
and relationships.In VG dataset, each image contains region descriptions that describe a localized portion of the image and question answer pairs, and each region is converted to a region graph representation of objects, attributes, and pairwise relationships, finally each of these region graphs are combined to form a scene graph with all the objects grounded to the image.VG contains over 108K images where each image has an average of 35 objects, 26 attributes, and 21 pairwise relationships between objects.


\noindent\textbf{VAW: }
VAW is a large-scale in-the-wild visual attribute prediction dataset based on the VGPhraseCut and GQA datasets, which aims to overcome the deficiency of VG dataset in attribute prediction task. VAW is composed of 72,274 images with 620 unique attributes including color, material, size, action and many others. VAW consists of 2260 objects observed in the wild and 260,895 instances of different objects with over 927K labeled positive and negative attribute annotations. Each attribute-object pair in VAW has at least 50 positive and negative annotations.


\noindent\textbf{SWIG: }
SWiG is a challenging dataset based on the large imSitu dataset, which adds 278,336 bounding-box groundings to the 11,538 entity classes.The SWiG dataset contains 126,102 images and 504 verbs in total. The bounding-box annotations of the images are obtained using Amazon's Mechanical Turk framework, and each role is manually annotated. SWiG contains a total of 451,916 noun slots, of which 63.9\% have bounding boxes. Objects that lack bounding-box annotations are invisible or performing an action that cannot be annotated.


\noindent\textbf{HAKE: }
To address and promote the ability to activity understanding in the field of deep learning, some researchers have constructed HAKE dataset. Human Activity Knowledge Engine (HAKE) is based on the human body part states. Based on the existing active datasets, the part stages of active persons in all images are annotated. This well establishes the relationship between instance activity and body part states. At present, 104 K+ images are annotated in the dataset, which includes 677 K+ human instances, 278 K+ interacting objects, 733 K+ instance actions, 7 M+ human body part states. 


==> experiments.tex <==
\subsection{Data Setup}
We used four corpora, VG~\cite{krishna2017visual}, SWiG~\cite{Pratt2020Swig}, VAW~\cite{Pham2021vaw} and HAKE~\cite{Li2019HAKEHA} to build benchmark dataset for each capability test in the proposed framework. Table~\ref{tbl:data-summary} is a summary.  Then, we adopt these corpora to create VL-CheckList evaluation with the following steps:

\textbf{Object: }
With regard to Object, the evaluation corpus is converted from SWiG, VG and HAKE datasets. We divide the Object into two evaluation indicators: Size and Location. The former focuses on the model's understanding of the size of the object in the picture, while the latter focuses on the model's attention to the location of the object in the picture. For example, for Location (Center), we select the object in the center of the picture(e.g. man riding on top of a \textbf{skateboard}) and replace it with another object(e.g. man riding on top of a \textbf{pilot}).

\textbf{Attribute: }
The evaluation corpus of Attribute is transformed from VG and VAW datasets. According to the attribute classification of VAW, we divide attribute into five evaluation metrics: Color, Material, Size, State and Action. Take Color as an example. For VAW datasets, positive samples are composed of subjects, copulations and corresponding colors(e.g. sheep is \textbf{white}), while negative samples replace the original colors with other colors(e.g. sheep is \textbf{golden brown}).

\textbf{Relation: }
For Relation, the evaluation corpus is converted from VG, SWiG and HAKE dataset. According to whether the predicate is a preposition or not, we divide Relation into Action and Spatial. Action can better reflect the model's understanding of advanced verbs, while spatial focuses more on the model's understanding of spatial relations. For Action, the positive samples consist of subject, predicate and object (e.g. child \textbf{brushing} teeth), while the negative sample replaces the predicate with \emph{verb-ing} (e.g. child \textbf{photographing} teeth). For Spatial, the negative sample replaces the predicate with prepositions (e.g. shirt \textbf{on} boy $\rightarrow$ shirt \textbf{under} boy).

==> results-backup.tex <==
In this section, we show the experiment results of the seven models based on the proposed framework.

\subsection{Overall Performance}
\begin{table}[ht]\centering
   
    \begin{tabular}{c|c|c|c}
    \hline
    Models & Object & Relation & Attribute \\
    \hline
        ViLT & \textbf{86.32} 	&62.50 	&76.96  \\
        ALBEF & 81.08 	&70.05 	&\textbf{77.95}  \\
        OSCAR & 84.41 	&\textbf{75.60} 	&76.68  \\
        UNITER & 81.94 	&71.25 	&71.45  \\
        LXMERT & 82.36 	&59.20 	&74.80  \\
        TCL & 81.58 	&63.45 	&76.06  \\
        CLIP & 82.93 	&58.60 	&64.37  \\
    \hline
    \end{tabular}
    \caption{Overall performance}
    \label{all}
\end{table}

Table \ref{all} shows the overall performance of the seven VLP models on the Object, Relation and Attribute evaluation metrics. Compared with Relation and Attribute, models obtain higher scores on the Object metric, which indicates that the models have a deeper understanding of object than relation and attribute. In terms of Object evaluation metric, the performance of the seven models is similar, and ViLT and OSCAR are a little better than others. The performances of models on Relation metric vary a lot. Oscar with the highest score is 16.4 points higher than LXMERT with the lowest score. On the attribute metric, the performance of CLIP is much worse than that of other models.

\begin{table*}
\centering
\begin{tabular}{c|c|ccc|ccc}
\hline
\multirow{2}{*}{Model}&\multirow{2}{*}{Average}&\multicolumn{3}{c|}{Size}&\multicolumn{3}{c}{Location}\\
\cline{3-8}
& & Large & Medium & Small & Center & Mid & Margin \\
\hline
    ViLT & \textbf{86.32} 	&88.58	&85.29	&\textbf{82.18} &\textbf{88.61} 	&\textbf{86.65}	&\textbf{86.59}\\
    ALBEF & 81.08 	&84.33	&80.25	&76.92 &82.87 	&80.91 	&81.19\\
    OSCAR & 84.41 	&88.41	&\textbf{85.40}	&78.92 &88.01 	&85.50 	&80.24\\
    UNITER & 81.94 	&85.27	&81.12	&78.06 &85.69 	&83.64 	&77.84\\
    LXMERT & 82.36 	&84.94	&82.05	&79.01 &84.56 	&83.84 	&79.77\\
    TCL & 81.58 	&86.15	 &79.96	 &74.91 &85.01 	&83.21 	&80.26\\
    CLIP & 82.93 	&\textbf{88.83}	&81.99	&75.70 &88.53 	&85.86 	&76.66\\
\hline
\end{tabular}
\caption{Evaluation of Object metric}
\label{obj}
\end{table*}


\begin{table*}
\centering
\begin{tabular}{c|cc|c|cc|c}
\hline
\multirow{2}{*}{Model Type}&\multicolumn{3}{c|}{Location}&\multicolumn{3}{c}{Size}\\
\cline{2-7}
& Center & Margin & Variance & Large & Small & Variance \\
\hline
    E2E & 85.50 	&82.68 	&2.82	&86.35 &78 &8.35 \\
    Region-based & 86.09 	&79.28 	&6.81 &86.2 &78.66 &7.54\\
    CLIP & 88.53 	&76.66 	&\textbf{11.87} &88.83 &75.70 &\textbf{13.13}\\
\hline
\end{tabular}
\caption{The variance of three types of models in Location and Size. E2E means end-to-end models, which are ViLT, ALBEF and TCL in our paper, while Region-based means OSCAR, UNITER and LXMERT, and finally a CLIP. All numbers in table represent the average score.}
\label{Loc}
\end{table*}

Table \ref{obj} demonstrates the influence of different size and location on the performance of models. Specifically, we observe all models gain the highest scores in Large and Center, which shows that VLP models tend to focus on larger objects and those in central point. Particularly, CLIP has the most performance degradation when it's from Large to Small and Center vs. Margin(13.13\% and 11.87\% degradation, respectively). Moreover, end-to-end models(ViLT, ALBEF and TCL) are more stable in Location variance than others. Their scores dropped by an average of only 2.82\% from Center vs. Margin, compared with an average of 6.8\% for region-based models(OSCAR, UNITER and LXMERT) and 11.87\% for CLIP.
    
\begin{table}[ht]\centering    
    \begin{tabular}{c|c|cc}
    \hline
    \multirow{2}{*}{Model}&\multirow{2}{*}{Average}&\multicolumn{2}{c}{Relation}\\
    \cline{3-4}
    & & Action & Spatial \\
    \hline
    ViLT & 62.50	&56.90	&68.10\\
    ALBEF & 70.05	&67.10	&73.00\\
    OSCAR & \textbf{75.60}	&\textbf{71.60}	&\textbf{79.60}\\
    UNITER & 71.25	&67.50	&75.00\\
    LXMERT & 59.20	&55.00	&63.40\\
    TCL & 63.45	    &59.20	&67.70\\
    CLIP & 58.60	&56.50	&60.70\\
    \hline
    \end{tabular}
    \caption{Evaluation of Relation metric}
    \label{relation}
\end{table}

Table \ref{relation} shows the performance of the models on Relation metric. Relation consists of Action and Spatial. The former focuses on complex verbs and the latter on spatial relations. It can be seen from the table that the score of the model on Action is generally lower than that of Spatial. It can be concluded that it is easier for models to understand spatial relationships than complex verbs.Oscar performs best in both Action and Spatial. It seems that Oscar is better at handling relationship than other models.
    
\begin{table*}[ht]\centering    
    \begin{tabular}{c|c|ccccc}
    \hline
    \multirow{2}{*}{Model}&\multirow{2}{*}{Average}&\multicolumn{5}{c}{Attribute}\\
    \cline{3-7}
    & & Color & Material & Size &State &Action \\
    \hline
    ViLT & 76.96	&\textbf{87.80}	&83.45	&67.30	&70.70	&75.55\\
    ALBEF & \textbf{77.95}	&85.40	&\textbf{85.30}	&64.65	&\textbf{74.95}	&\textbf{79.45}\\
    OSCAR & 76.68	&82.70	&84.30	&64.80	&72.94	&78.65\\
    UNITER & 71.45	&78.10	&75.75	&63.05	&67.70	&72.65\\
    LXMERT & 74.80	&83.40	&80.05	&\textbf{67.95}	&67.59	&75.00\\
    TCL & 76.06	    &84.00	&84.00	&61.95	&74.15	&76.20\\
    CLIP & 64.37	&65.15	&66.70	&59.80	&66.08	&64.10\\
    \hline
    \end{tabular}
    \caption{Evaluation of Attribute metric}
    \label{attr}
\end{table*}



Table \ref{attr} shows the performance of the models on Attribute metric. Attribute includes Color, Material, Size, State and Action. As can be seen from the table, the models score relatively well on Color and Material, while poor on Size, State and Action, and the models perform worst on Size. Compared with other models, CLIP has the lowest score on all metrics of Attribute.

\subsection{Analysis}
Based on the results we obtained, we conduct further analysis and extension experiment in this section.  

\subsubsection{Analysis about CLIP model}
In this section, we discuss the fastest degradation of CLIP performance in (Large to Small) and (Center to Margin), as well as the reasons for the poor results of Attribute:

\textbf{Center vs. Margin}:
From Table \ref{obj}, it can be seen that the gap score between Center and Margin of CLIP model is 11.87\%, which is one of the largest average contrast fluctuation among all models. Appendix Table \ref{clip_good} shows that the results of CLIP on SWiG and HAKE are good, but the results in VG dataset are poor. We guess that the CLIP model itself has limited ability to understand the semantic information of complex scenes. In the pre-trainning stage, it calculates the feature similarity according to a piece of text and an image, but region base model uses the external convolution architecture to extract region targets from images, and end-to-end model makes better use of attention mechanism to learn the similar fraction of image-text in the feature fusion stage. The above method, which is different from CLIP, may be better than calculating the similarity using the feature matrix alone. By contrast, in the aspects of cross modal feature fusion, attention mechanism can better insight into objects with smaller area. In order to test this hypothesis, we did an extension experiment of CLIP on the location-related datasets. Each data item of VG provides \textbf{'region-info'} label, including the bounding box of the image regions of \textit{subj} and \textit{obj}. Therefore, we integrate two bounding boxes into a matrix box, extract the image regions, and keep the description text in the sample unchanged to form a new image-text pair \textbf{(Image$_{local}$,text)}, and constructed variant datasets for VG: Local$_{subj}$, Local$_{obj}$. The results of the supplementary experiment are shown in Table \ref{clip_local} . We see that by removing as much of the edge information that is independent of the single-segment text description as possible from the image, the results of CLIP for local image on Local$_{subj}$ and Local$_{obj}$ are outperformed the original CLIP (no image region is extracted), 3.9\% and 5.7\% higher respectively. The results were even better than the region base multimodal models. The table \ref{obj} shows that multimodal models generally pay more attention to the central semantic information of images, which is similar to the perspective of human observation. Focusing on the image region will improve the ability of CLIP model to obtain more fine-grained visual signals. We believe that the sensitivity of CLIP to scene location information is a work worthy of further study.


\textbf{Large vs. Small}:
 We further measure how the pixel size of the region in the image will affect the model. The variance value of CLIP from the small and large region images is the largest, which is 13.13\% degradation. The region base and end to end models are more stable, even if the other six models are used for single comparison, the conclusion is still the same. This is not only due to the absence of attention mechanism in feature similarity computing. CLIP was trained to match an image as a whole to a text description, without capturing the fine-grained alignment between image regions and text spans, so the understanding of local information is not very good ~\cite{zhong2022regionclip}.
 
 \textbf{Poor Attribute}:
 Table \ref{attr} shows that the ability of CLIP to understand attribute related visual commonsense was poor, which is more prominent than other models. Whether it is the influence of neural network structure difference or the training data is also a work worth discussing in the future.


\subsubsection{Analysis about Location}
Table \ref{Loc} shows the performance degradation of two types of models on Location variance. It is obvious that end-to-end models are more stable than region-based models, which we speculate that is because self-attention mechanism on a full image can help VLP models focus flexibly on any area of an image even it is located in somewhere unclear while the visual features of region-based models are usually extracted by object detector(\textit{e.g.} Faster R-CNN) so that these models depend on the performance of object detector and can only pay attention to those regions extracted by it but not all areas of an image. Moreover, that located in the margin of the image may be incomplete which object detector tend to ignore thus it can't offer corresponding visual information to VLP models. Therefore, region-based models is prone to miss some useful information located in the margin. We generate the heat-maps of two types of models for some same images to evidence our hypothesis, and we show two of them in Figure \ref{fig:heat-map-car} and Figure \ref{fig:heat-map-pants}.

As shown in Figure \ref{heat-map-car-a}, its descriptive text is: wheel ON \textit{car}, and \textit{car} is the word replaced in the negative sample, that is what we expect model to focus on. But we can observe from Figure \ref{heat-map-car-b} that object detector fails to get the region proposal of the \textit{car} on the top of image as a result of its incomplete display , which leads to region-based model miss the object \textit{car} while end-to-end model focus accurately on this region, as shown in Figure \ref{heat-map-car-c} and \ref{heat-map-car-d}. Another example is described in Figure \ref{fig:heat-map-pants}, whose descriptive text is: boy has \textit{pants}, and \textit{pants} is the replaced word. Figure \ref{heat-map-pants-b} illustrates that object detector fail to get the proposal of the \textit{pants} because it's incomplete and unclear. It's easy to observe from Figure \ref{heat-map-pants-c} and \ref{heat-map-pants-d} that region-based model can't catch the \textit{pants} while end-to-end model recognizes it successfully. It deserves to be mentioned that ALBEF judged correctly about both of above two images in ITC task while OSCAR and LXMERT failed.



\begin{figure*}
\centering
\subfigure[]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=1.1in]{images/heatmap/car.jpg}\\
%\caption{fig1}
\label{heat-map-car-a}
\end{minipage}%
}%
\subfigure[]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=1.1in]{images/heatmap/car_bb.jpeg}\\
%\caption{fig2}
\label{heat-map-car-b}
\end{minipage}%
}%
\subfigure[]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=1.1in]{images/heatmap/car_lxmert.png}\\
%\caption{fig2}
\label{heat-map-car-c}
\end{minipage}
}%
\subfigure[]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=1.1in]{images/heatmap/car_albef.jpg}\\
%\caption{fig2}
\label{heat-map-car-d}
\end{minipage}
}%
\centering
\caption{\textbf{(a).}The original image, its descriptive text is: 'wheel ON \textit{car}'. \textbf{(b).}The bounding boxes extracted by Faster-RCNN. \textbf{(c).}The heat-map of LXMERT for the word \textit{car}. \textbf{(d).}The heat-map of ALBEF for the word \textit{car}.}
\label{fig:heat-map-car}
\end{figure*}



\begin{figure*}
\centering
\subfigure[]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=1in]{images/heatmap/pants.jpg}\\
%\caption{fig1}
\label{heat-map-pants-a}
\end{minipage}%
}%
\subfigure[]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=1in]{images/heatmap/pants_bb.jpeg}\\
%\caption{fig2}
\label{heat-map-pants-b}
\end{minipage}%
}%
\subfigure[]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=1in]{images/heatmap/pants_oscar.png}\\
%\caption{fig2}
\label{heat-map-pants-c}
\end{minipage}
}%
\subfigure[]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=1in]{images/heatmap/pants_albef.jpg}\\
%\caption{fig2}
\label{heat-map-pants-d}
\end{minipage}
}%

\centering
\caption{\textbf{(a).}The original image, its descriptive text is: 'boy has \textit{pants}'. \textbf{(b).}The bounding boxes extracted by Faster-RCNN. \textbf{(c).}The heat-map of OSCAR for the word \textit{pants}. \textbf{(d).}The heat-map of ALBEF for the word \textit{pants}.}
\label{fig:heat-map-pants}
\end{figure*}



\subsubsection{Analysis about Relation}
In this section, we group seven models by the number of their layers of multimodal-encoder, which makes the conjunction of semantic features and visual features as input and apply cross-attention to it, and calculate their average scores about Relation. As shown in Figure \ref{fig:layer-relation}, we observe that their performance about Relation increase as their number of layers increases. We conjecture that more layers of multimodal-encoder can help VLP models learn relation better, which is high-level semantic information and hard to learn well. Similar viewpoint has been put forward by \cite{tenney2019bert}, which found high-level semantic information appears and be captured at higher layers of BERT, whose achievement on single modality of language makes our analogous hypothesis on multimodal more convincing. Another observation is that CILP, which has no multimodal encoder, is just slightly weak than LXMERT on Relation, even outperforms on Action a little(Figure \ref{relation}). We guess ... .Above conjectures are promising to be evidenced and we leave deeper understanding as future work.

Also, we generate some heat-maps to show where VLP models focus about Relation, as shown in Figure \ref{fig:heat-map-working}. The descriptive text of the image is: the woman is \textit{working} on her computer at desk, and we generate the heat-maps of four different models for the word \textit{working}. Generally, human will focus on the region that the woman typing on keyboard with hand when it comes to the word \textit{working}. Therefore, OSCAR and ALBEF get right, while LXMERT doesn't pay enough attention (the proposal including hand and keyboard is less clear than OSCAR) though it find right region and the area focusd by ViLT is not so accurate.



\begin{figure}
\centering
\includegraphics[scale=0.4]{images/relation.jpg}
\caption{The performance of VLP models with different number of multimodal-encoder layers.OSCAR and UNITER have 24 layers of multimodal-encoder, ViLT, ALBEF and TCL have 12 layers, LXMERT has 5 layers and CLIP has no multimodal-encoder layers. It can be observed that their average scores about Relation is also in this order from Table \ref{relation}}
\label{fig:layer-relation}
\end{figure}


\begin{figure*}
\centering
\subfigure[]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=1.2in]{images/heatmap/working_oscar.png}\\
%\caption{fig1}
\label{heat-map-car-a}
\end{minipage}%
}%
\subfigure[]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=1.2in]{images/heatmap/working_lxmert.png}\\
%\caption{fig2}
\label{heat-map-car-b}
\end{minipage}%
}%
\subfigure[]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=1.2in]{images/heatmap/working_albef.jpg}\\
%\caption{fig2}
\label{heat-map-car-c}
\end{minipage}
}%
\subfigure[]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=1.2in]{images/heatmap/working_vilt.png}
%\caption{fig2}
\label{heat-map-car-d}
\end{minipage}
}%
\centering
\caption{The heat-map for the word \textit{working} of OSCAR, LXMERT, ALBEF and ViLT, respectively}
\label{fig:heat-map-working}
\end{figure*}



\begin{table}[ht]\centering    
    \begin{tabular}{c|c|c|c|c}
    \hline
    Model\ \textbf{\textbackslash{}}\ VG$_{data\_type}$ &Subj &Obj &Local$_{subj}$ &Local$_{obj}$\\
    \hline
    ViLT & \textbf{89.3}	&\textbf{95.1}	&-	&- \\
    ALBEF & 87.8	&93	&-	&- \\
    OSCAR & 83.9	&84.7	&-	&- \\
    UNITER & 84.8	&86.4	&-	&- \\
    LXMERT & 84.3	&86.8	&-	&- \\
    TCL & 85	&91.1	&-	&- \\
    CLIP & 80.7	&86	&-	&- \\
    CLIP\_Local & -	&-	&\textbf{84.6}	&\textbf{91.7} \\
    \hline
    \end{tabular}
    \caption{Subj and Obj are two attribute subsets extracted from VG dataset. Using the bounding box tag of VG to merge and extract the region image pointed by \textit{subj} and \textit{obj} fields, a new dataset is constructed. The text remains the same as previous content \textbf{(Image$_{local}$,text)}. It only does the expansion experiment for CLIP.}
    \label{clip_local}
\end{table}









% - overall performance
% Table, Rader etc. 

% - dual encoder vs cross/merged attention
% CLIP
%   - CLIP is good at some data, but poor in other (VG)
%   - Study -> region + CLIP
%     - New Table
%     - explanation: why CLIP fail on VG
%     - picture

% - location (region vs e2e)
%   - center/margin variance is small?
%   - table or Figure (diff graph)
%   - qualitative heat-map example
 
% - relation (OSCAR, CLIP)
%   - Table (Action < Spatial) VG
%   - breakdown table (show high-performance models)
%   - ?? 
 
%  - Attribute
%   - all models not good for linguist size (small vs large)
%   - potential research direction.













